Physics with Reactor Neutrinos

Neutrinos produced by nuclear reactors have played a major role in advancing our knowledge of the properties of neutrinos. The first direct detection of the neutrino, confirming its existence, was performed using reactor neutrinos. More recent experiments utilizing reactor neutrinos have also found clear evidence for neutrino oscillation, providing unique input for the determination of neutrino mass and mixing. Ongoing and future reactor neutrino experiments will explore other important issues, including the neutrino mass hierarchy and the search for sterile neutrinos and other new physics beyond the standard model. In this article, we review the recent progress in physics using reactor neutrinos and the opportunities they offer for future discoveries.

==> Makefile <==
########################################################################
#
# $Id: Makefile,v 1.2 2010/10/29 15:06:33 slavic Exp $
#
##########################################################################
TEX = pdflatex
BIB = bibtex
#main file
texfile = reactor_physics
#all figures
FIGS=$(wildcard figures/*.*)
#all texfiles
SECS=$(wildcard ./*.tex)
#SECS=$(wildcard sections/*.tex)

export TEXINPUTS:=$(CURDIR):$(CURDIR)/ar2estyle:$(TEXINPUTS)
export BSTINPUTS:=$(CURDIR):$(CURDIR)/ar2estyle:$(BSTINPUTS)
export BIBINPUTS:=$(CURDIR):$(CURDIR)/ar2estyle:$(BIBINPUTS)

.PHONY: pdf
.PHONY: clean

all: pdf

pdf: $(texfile).pdf

$(texfile).pdf : $(SECS) $(texfile).tex $(texfile).bib #$(FIGS) 
	$(TEX) $(texfile)
	$(BIB) $(texfile) # compile bibliography
	$(TEX) $(texfile)
	$(TEX) $(texfile)

clean:
	@ls $(texfile).* | grep -v '.tex\|.bib' | xargs -I {} rm {}

